A Survey on Predictive Maintenance for Industry 4.0

Production issues at Volkswagen in 2016 lead to dramatic losses in sales of up to 400 million Euros per week. This example shows the huge financial impact of a working production facility for companies. Especially in the data-driven domains of Industry 4.0 and Industrial IoT with intelligent, connected machines, a conventional, static maintenance schedule seems to be old-fashioned. In this paper, we present a survey on the current state of the art in predictive maintenance for Industry 4.0. Based on a structured literate survey, we present a classification of predictive maintenance in the context of Industry 4.0 and discuss recent developments in this area.

==> kapitel/Abbreviations.tex <==
%-------------------------------------
%
%    minimales abk�rzungsverzeichnis
%
%-------------------------------------

%\addchap{Abk\"{u}rzungsverzeichnis} % beachte addchap
\addchap{List of Abbreviations}
\begin{labeling}{1234567890}
    
        \item[ARFF]Attribute-Relation File Format
        \item[CPS] Cyber-Physical System
        \item[CRISP-DM] Cross-Industry Standard Process for Data Mining
        \item[CSV] Comma-Separated Values
        \item[IIoT] Industrial Internet of Things
        \item[IoT] Internet of Things
        \item[MLA] Machine Learning Algorithm
        \item[PM] Predictive Maintenance
        \item[SLR] Structured Literature Review
        \item[WEKA] Waikato Environment for Knowledge Analysis

\end{labeling} 



==> kapitel/Conclusion.tex <==
\section{Conclusion}
\label{chap:conclusion}
The present survey represents a comprehensive analysis of the topic of Predictive Maintenance (PM). PM distinguishes itself from conventional maintenance policies by the attempt to not solely detect an anomaly of a machine or component, but to predict when the failure might occur in order to efficiently schedule maintenance actions in advance. Researchers are severely interested in the concept of PM since hundreds of papers with regard to the topic are published every year. Minimized downtime, prolonged machine life, increased productivity and reduced costs are merely a few promising prospects of PM. The objective of the present survey is to detect and categorize a variety of aspects with regard to the comprehensive topic of PM. For the purpose of the survey 150 papers are analyzed and categorized. The result is a data grid with 69 attributes which are clustered into the following 10 categories: Goals, Condition Monitoring, Maintenance Scope, Degradation Process, Fault Detection, System Size, Scheduling, Prognostic Techniques, Data Handling and Evaluation. These 10 categories together with their corresponding attributes built a framework for PM. Additionally a machine learning analysis with WEKA is conducted in order to reveal presumable connections between attributes and categories of the framework.


	\subsection{Reflection of the Procedure}
	\label{sec:reflection}
For the present survey a structured literature review (SLR) is conducted. This approach is beneficial in contrast to the berry picking method as it captures all facets of the topic. Since the objective of the present survey is to categorize and structure a comprehensive scope of the research field of PM, the SLR is the more appropriate choice. In order to construct the framework for PM, the 150 papers are analyzed and categorized which results in 10 categories and 69 attributes each belonging to one category. Although the number of papers in the research field of PM ranges into the thousands, the number of papers in this survey represents an informative cross subsection of the topic. Hence, the framework provides a comprehensive overview about PM. The concept of deducing attributes, grouping them into categories and building a framework related to a specific topic is very beneficial in order to get a structured and deeper understanding of a subject and to reveal potential gaps in the existing literature. Especially when analyzing a considerable number of scientific publications. Furthermore, the machine learning analysis allowed an even deeper understanding of the topic as it points out potential connections between attributes of the framework which might be difficult to detect otherwise. Generally, the procedures and methods of the present survey support the accomplishment of the predetermined objectives.   

	
	\subsection{Answering the Research Questions}
	\label{sec:answerquestions}
How can PM approaches be differentiated and classified? This first research question of the present survey is meant to structure the topic of PM. Considering that there haven been thousands of papers published over decades with regard to PM raised the question in which way the existing research can be classified in order to structure it and to reveal potential gaps for further research. The answer to this research question is presented in form of the PM framework. The framework structures and classifies papers published between 1993 and 2018. The  framework makes no claim of completeness, neither are the attributes within each category. Nevertheless, the framework of the present survey covers relevant aspects and facets of the topic of PM and builds a comprehensive introduction into the research field of PM.

Can machine learning algorithms improve the informational value of a survey? This second research question is based on the idea that the collected data of a survey might not solely be useful to structure the topic, but also to gain a deeper understanding about certain connections within the research field. The analysis with WEKA of the present survey shows that MLAs are in fact useful in order to analyze the literature data. Especially decision trees point out potential connections between attributes of the framework and thus might reveal relationships between categories as well. However, the interpretation of the results should be conducted cautiously as the algorithms can never reveal causality but merely statistical correlation.
	
	
	\subsection{Critical View and Recommendations for Future Research}
	\label{sec:criticalview}
The present survey structures the topic of PM and facilitates a deeper understanding of the topic. Nevertheless, the survey makes no claim of completeness. As the number of papers surveyed is merely a fraction of the academic literature addressing the topic of PM, the framework is presumably incomplete with regard to the number of categories and especially with regard to the corresponding attributes within each category. For example, the prognostic techniques in the framework of this survey are an extract of all the available techniques. Furthermore, the design of the machine learning analysis is only one possible solution. subsection \ref{sec:discussionmachine} states alternative designs for a downsized analysis based on attribute removal according to predefined hypotheses or minimum frequency thresholds.

The framework of the present survey shows that further research might be appropriate in certain directions of the topic. First, the effect of different types of machine and component dependencies in the context of multi-component systems. Second, remote data storage and access using IoT technology for remote PM approaches. Third, the relevance of data fusion and data filtering due to big data issues as a result of an increasing number of monitoring sensors. Finally, the possibilities for a less complex and more affordable implementation of PM systems even for small and medium sized companies. Note that these research gaps are presumed based on the result of the present survey which does not cover all the existing academic literature. 


==> kapitel/Discussion.tex <==
\section{Discussion}
\label{chap:discussion}
The previous chapters covered the detailed structure of the PM framework as well as the machine learning analysis of the data derived throughout the literature review of academic articles. The following chapter will discuss the findings and procedures of these previous parts by developing hypotheses which additionally support answering the research questions in subsection \ref{sec:answerquestions}. Chapter \ref{chap:discussion} is divided into two parts. First, subsection \ref{sec:discussionframe} focuses on the PM framework and discusses potential gaps in the academic literature and the connection to the topic of Industry 4.0. Second, subsection \ref{sec:discussionmachine} discusses whether a machine learning analysis is beneficial for this type of survey. 


\subsection{Discussion of the Framework}
\label{sec:discussionframe}
The number of papers analyzed in the present survey is merely a fraction of the available academic literature addressing PM. However, the analysis provides insides about which aspects the literature mostly focuses on. This discussion concentrates on four aspects that emerged during the construction and analysis of the PM framework. First, an interesting aspect in this context is the topic of dependencies. Although 41 papers state that they take multi-component systems into account, merely 8 papers address the topic of dependencies. This implies that although PM is more efficient when applied to an entire production system instead of single machines and when taking dependencies into consideration, the existing literature frequently focuses on a too narrow view on PM. Many researchers either apply their approach merely to a single machine or they do not focus on dependencies of any of the three types described in subsection \ref{sec:systemsize}. Nonetheless, dependencies are severely important when attempting to design an efficient and integrated PM system which can be applied to an entire manufacturing process. Thus, in this area seems to be a gap in the existing research and further research should focus on a broader scope for PM systems.

Second, to date a minority of papers address modern possibilities of remote data storage and remote data access. However, with the available technology and improving internet connections for a faster transfer of data, future PM approaches should use these technologies more severely in order to create a more centralized, networked and therefore more efficient PM system. This is especially of interest for companies with multiple manufacturing locations. When all the information can be accessed and processed at a remote location for every manufacturing site, resources can be distributed more efficiently. Furthermore, production facilities only need to install the sensor technology for monitoring and data collection purposes as the data processing is conducted remotely. Hence, connecting multiple locations to a centralized PM system has the potential to create economies of scale. Nevertheless, since PM is not simply scalable for any system size \cite{Nguyen2015}, the centralized system needs to take into account structural, stochastic and especially economic dependencies. Hence, with regard to an implementation of PM in the context of Industry 4.0 remote data storage and access should come to the fore of further research.

The third aspect which might point out a gap in the existing research based on the sample of papers analyzed in the present survey is related to the category of data handling as well (see subsection \ref{sec:datahandling}). Hardly over 20 papers address the topic of data fusion and data filtering. This might be the case since a lot of research focuses on single-component systems. However, with an increasing number of sensors in use the amount of data increases and makes methods such as data fusion and data filtering necessary in order to process it efficiently. Especially in an Industry 4.0 environment with multiple integrated systems, big date becomes an issue. PM systems not only generate an increasing amount of data because of multiple machines or even multiple manufacturing locations but additionally due to improvements in sensor technology which will allow to monitor even more parameters then before. Wireless sensors already enable the collection of monitoring data where it was not possible to collect data before due to fragile wires. The improvements in sensor technology will support PM systems in becoming more accurate. Nevertheless, in order to keep PM systems efficient with regard to processing power usage and big data, further research is needed in the area of feasible methods of data filtering and data fusion.  

Finally, no paper in the present survey covered the topic of possibilities for small and medium sized companies. The research shows opportunities of PM such as cost minimization, increased productivity and prolonged machine life. However, none of the papers in the present survey address the issue of how firms can implement a PM system in a cost minimizing way. Thus, while the latest sensor and data processing technology might be affordable for large companies due to economies of scale, since one PM system can process data of multiple sensors, small and medium sized companies are unlikely to implement a PM system due to high upfront costs and complexity \cite{Carnero2006}. Nonetheless, the majority of firms are small and medium sized companies. The researchers show what is possible and do not focus on what is practical and can be implemented on a broad scale in order to boost an economies productivity and use of resources. Therefore, further research should focus on developing PM systems that are simple and affordable to implement even for smaller companies.

To sum it up, the present survey reveals research gaps  in the context of Industry 4.0. The research often focuses on too narrow aspects instead of more broader concepts as it would be necessary in an Industry 4.0 environment. The connection of PM systems to other processes such as spare part logistics should be considered in further research. Hence, the PM system should be addressed as part of a larger integrated system. Furthermore, possibilities for a large scale implementation are an issue as the literature shows what is possible, but only few companies have yet successfully implemented a PM system \cite{Efthymiou2012}.  


\subsection{Discussion of the Machine Learning Analysis}
\label{sec:discussionmachine}
The following subsection discusses the feasibility and utility of MLAs for surveys. While the framework showed presumable gaps in the existing literature, the objective of the machine learning analysis is to reveal relations between attributes and to reinforce hypotheses about attribute connections. Hence, the number of appropriate MLAs for classification is limited. The analysis of the present survey focuses on the OneR and J48 algorithm and the baseline accuracy (ZeroR). Although the two algorithms are basically the opposite of each other, they both help to achieve the survey's objective. The OneR algorithm works very simple and attempts to best explain or predict the tested attribute with just one other attribute. Thus, this algorithm shows a potential one on one attribute relation. However, one should be cautious as the algorithm might find the best fit in absolutely implausible attribute pairs. An example for such an implausible relation is shown in subsection \ref{sec:oner}. On the other hand, the J48 algorithm considers all attributes for its model and generates a decision tree with the most relevant attributes at the top. Hence, the J48 algorithm's output is more complex to interpret but at the same time it is more informative, robust and reliable compared to the OneR algorithm. Nevertheless, it is possible that the J48 algorithm generates a tree which merely consists of the OneR attribute and therefore does snot reveal any further information. As already mentioned in subsection \ref{sec:j48} the OneR algorithm can function as a first indication for a possible attribute relation but a detailed evaluation always requires the more complex J48 algorithm analysis.

As shown in subsections \ref{sec:oner} and \ref{sec:j48} MLAs are a great tool which can provide additional information about the acquired data which would be hard and time-consuming or even impossible to deduce otherwise. However, when covering a broad topic such as PM and analyzing 150 or more academic papers with different research interests and focuses within the same topic, the number of attributes relative to the number of instances can become very high. In the present survey with 150 instances 69 attributes where discovered during the SLR. Thus, even for two algorithms the number of runs including the ZeroR algorithm goes up to over 210. The issue with the number of runs is that it is very time-consuming to evaluate all the outcomes of the analysis in detail. Especially with large decision trees the evaluation for all attributes will take time. In particular attributes which appear only in a few instances might create larger trees without increasing the value of the tree since these attributes might be unlikely to imply a relation because of their negligible occurrence in the sample. Therefore, the present survey evaluates merely a few attributes in order to demonstrate how a detailed evaluation of an attribute can be conducted. Furthermore, the survey provides all the necessary data to conduct these evaluations. Hence, the results of the present survey support the understanding of PM and the relations between attributes within the topic. However, an important lessons learned of the present survey is that if a survey's objective is to focus on the evaluation of the machine learning analysis, the algorithms should not be applied to a data set containing all attributes found during the SLR. One method could be to create multiple smaller data sets which consists of only a selection of all the categories, e.g. condition monitoring and data handling. The selection should always be based on a preceding hypothesis. Another method to reduce the number of runs and in particular the size and complexity of the decision trees might be to define a lower bound for the frequency of occurrence. This means that only attributes which appear at least in as many instances as the lower bound become part of the data set for the machine learning analysis. Thereby, the analysis will be downsized to a level where the scope of the survey allows a detailed evaluation of all tested attributes and their relations to other attributes of the topic. 


==> kapitel/Erklaerung.tex <==
%% Auf der ersten rechten Seite soll unten das folgende stehen
\thispagestyle{empty}
\begin{center}
\begin{minipage}{14cm}
\thispagestyle{empty}


\vspace{6cm} \textbf{Eidesstattliche Erkl\"{a}rung:} 

Hiermit versichere ich, dass diese Arbeit von mir pers\"{o}nlich verfasst wurde und dass ich keinerlei fremde
Hilfe in Anspruch genommen habe. Ebenso versichere ich, dass diese Arbeit oder Teile daraus weder von mir
selbst noch von anderen als Leistungsnachweise andernorts eingereicht wurden. W\"{o}rtliche oder sinngem\"{a}�e
\"{U}bernahmen aus anderen Schriften und Ver\"{o}ffentlichungen in gedruckter oder elektronischer Form sind
gekennzeichnet. S�mtliche Sekund�rliteratur und sonstige Quellen sind nachgewiesen und in der Bibliographie
aufgef\"{u}hrt. Das Gleiche gilt f�r graphische Darstellungen und Bilder sowie f�r alle Internet-Quellen. Ich
bin ferner damit einverstanden, dass meine Arbeit zum Zwecke eines Plagiatsabgleichs in elektronischer
Form anonymisiert versendet und gespeichert werden kann. Mir ist bekannt, dass von der Korrektur der Arbeit
abgesehen werden kann, wenn diese Erkl\"{a}rung nicht erteilt wird
\\
\\
\textbf{English version (not legally binding):}

I hereby declare that the paper presented is my own work and that I have not called upon the help of a third
party. In addition, I affirm that neither I nor anybody else has submitted this paper or parts of it to obtain
credits elsewhere before. I have clearly marked and acknowledged all quotations or references that have
been taken from the works of others. All secondary literature and other sources are marked and listed in the
bibliography. The same applies to all charts, diagrams and illustrations as well as to all Internet resources.
Moreover, I consent to my paper being electronically stored and sent anonymously in order to be checked
for plagiarism. I am aware that if the declaration is not made, the paper may not be graded.
\vspace{2cm}\\
Mannheim, \today \hspace{2cm} Tim Wagenhals
\end{minipage}
\thispagestyle{empty}
\end{center}




==> kapitel/Foundations.tex <==
\section{Foundations of Predictive Maintenance}
\label{chap:foundations}
The following chapter covers the foundations and basics of PM. Section \ref{sec:iot} and \ref{sec:i4.0} place PM in the context of Internet of Things (IoT) and Industry 4.0. These concepts are briefly described and help to understand the importance and the variety of application possibilities for a PM approach. Section \ref{sec:predicmaint} introduces the topic of PM itself and its similarities and differences with conventional maintenance policies. Additionally, the modern integrated concept of e-maintenance is described in this section. Finally, section \ref{sec:machinelearn} briefly explains the basics of machine learning concepts and algorithms. 


	\subsection{Internet of Things (IoT)}
	\label{sec:iot}
The first step in digital integration of hardware are Cyber-Physical Systems (CPS). CPSs are the connection of a hardware and a software which is capable to describe the status of the corresponding hardware via installed sensors \cite{Cps10}. A mere CPS set-up would be sufficient to apply PM. However, the set-up is isolated from other CPSs and thus not optimal. Hence, IoT takes the concept of CPS to the next level by connecting multiple physical systems via internet with each other to form a complex network structure which allows coordinated activities \cite{Iot14}. In the context of production and maintenance this results in a more efficient and remotely controllable PM strategy for optimal resource allocation. The integration of IoT in the maintenance strategy is covered in section \ref{subsec:e-maint} which describes the concept of e-maintenance.

Since an integrated approach of IoT requires the upload of data via the internet, the machinery of a production facility needs to be monitored by sensors able to upload the acquired data. Nowadays, as communication technology is on the rise, wireless sensors are available which are capable of continuously monitoring machinery parameters while the machines are online and running \cite{Hashemian2011}, \cite{Hashemian2011a}. Additionally, as these modern sensors do not require any fragile physical connections by wires they are much more robust and can be used in more extreme environments \cite{Hashemian2011}, \cite{Hashemian2011a}. 		


	\subsection{Industry 4.0}
	\label{sec:i4.0}
Industry 4.0 is associated with the fourth industrial revolution. It combines technologies such as CPSs, IoT and cloud computing. The term was originally characterized by the German government. While the term Industry 4.0 is mostly used in the European area the term Industrial Internet of Things (IIoT) is an equivalent and also describes advances in big data, cloud computing and networking of machinery and systems in the industrial sector \cite{Jeschke2017}. 

Applying the concepts of CPSs and IIoT all necessary manufacturing processes including logistics, services and of course maintenance can be efficiently synchronized \cite{Lee2015}. In that sense, Industry 4.0 is an extension of mere CSPs and IoT as it does not focus on a single process such as maintenance but does also integrate other processes such as logistics for spare-parts and production materials \cite{Lee2015}. Thus, developing a highly flexible and entirely integrated optimized manufacturing process even with several companies involved. 

The complete implementation of Industry 4.0 or IIoT would result in a vision which is called smart factory. The smart factory is an integrated production process including logistic systems and even maintenance scheduling that is entirely self-organizing by the connected machines and intelligent software without any human interaction \cite{Smartfactory16}. Thus, allowing the cost efficient manufacturing of highly individual products \cite{Smartfactory16}. 


	\subsection{Predictive Maintenance}
	\label{sec:predicmaint}
The approach of PM was already introduced in chapter \ref{chap:introduction} as a maintenance policy leading to improved efficiency since it allows an estimation of the remaining useful life of the machinery. This approach is based on condition monitoring ideally conducted by sensors, which allows a continuous monitoring process of relevant machine parameters such as vibration and temperature. However, condition monitoring in isolation cannot be considered predictive as it only allows to identify the parameter changes that occur before a failure, but it does not allow to predict a relatively narrow future period of time in which the parameter changes happen and thus the failure might occur. Thus, it does not enable those responsible to schedule maintenance activities ahead in an efficient way, such as finding the most cost efficient time frame for shutting down the production process for maintenance activities. Consequently, a reliable prognostic technique is necessary to transform the acquired data into valuable information for failure prediction. Hence, prognostic techniques are an important part of PM and will be an important component of the PM framework in chapter \ref{chap:framework}.

In order to clearly differentiate PM from traditional conventional maintenance policies section \ref{subsec:maintpol} describes the most relevant categories of maintenance policies and their unique characteristics. Finally, section \ref{subsec:e-maint} briefly explains the modern approach of e-maintenance which integrates PM into a broader context of manufacturing processes.

		\subsubsection{Conventional Maintenance Policies}
		\label{subsec:maintpol}
Generally, maintenance policies can be divided in 2 categories: Corrective maintenance and preventive maintenance. A categorization of conventional maintenance policies is shown in figure \ref{img:maintenancepolicies}. Corrective maintenance always takes place after a failure occurred. Afterwards, the repairing of the machine can be done immediately or at some later point. A production plant that uses this approach is following a \emph{run-to-failure} management based on the philosophy: \emph{If it ain't broke, don't fix it} \cite{Mobley02}. However, this approach can result in severe reduction of manufacturing time ad costly repairs. Corrective maintenance is also referred to as reactive maintenance \cite{Mobley02}. On the other hand, preventive maintenance policies, also called proactive maintenance, are attempted to be executed before a fatal failure occurs. Thereby, preventive maintenance policies are divided into two categories. First, preventive maintenance where the maintenance activities are conducted on pre-scheduled intervals based on historic average equipment lifetime \cite{Schmidt2018}. On the contrary, condition-based maintenance monitors the current condition of a machine and schedules maintenance activities based on the observations made \cite{Schmidt2018}. Here, three distinct condition monitoring methods are feasible: Monitoring on request, scheduled monitoring and continuous monitoring \cite{Grall2002}, \cite{Zhou2007}. The first two methods are mostly based on inspection, while continuous monitoring is generally implemented by sensors. The drawbacks of predetermined maintenance were already discussed in section \ref{sec:improvements}. The issue with condition-based maintenance is that even with continuous monitoring the acquired data only represents a snapshot of a machines condition. The approach does not allow to efficiently schedule maintenance activities ahead due to missing knowledge about a machine's or component's presumable future state. However, as has already been mentioned and is shown in figure \ref{img:maintenancepolicies} the approach of PM is based on the idea of condition monitoring. Hence, PM represents an enhancement of mere condition-based maintenance.

\begin{figure}
	\centering
	\includegraphics[width=\textwidth]{figures/maintenancepolicies.png}
	\caption{Maintenance Policies \cite{Schmidt2018}}
	\label{img:maintenancepolicies}
\end{figure}

	
		\subsubsection{E-Maintenance}
		\label{subsec:e-maint}
Mere predictive maintenance is already an improvement in contrast to conventional maintenance policies. Nevertheless, a PM strategy which is carried out in isolation of other relevant processes still has potential for optimization. Hence, according to \cite{Lee2006} the efficiency can be severely improved by connecting multiple machines across manufacturing locations of a production facility and monitoring them remotely with wireless sensors, as described in section \ref{sec:iot}. A web application and cloud-based monitoring infrastructure allows to synchronize the process of maintenance with the overall operation even across production facilities. Furthermore, connected processes such as maintenance resources and even automated spare-part ordering can be integrated in this system \cite{Lee2006}. Precondition for such an e-maintenance system is to aquire and process relevant data in real time. \cite{Muller2008} argue that an e-maintenance can bee seen as an entirely integrated system since it handles the monitoring, diagnosis, prognosis and control process. Thus, e-maintenance goes beyond mere PM \cite{Lee2006}. To sum it up, the integrated approach of e-maintenance matches the concept and idea of Industry 4.0 covered in section \ref{sec:i4.0}.
		

	\subsection{Machine Learning}
	\label{sec:machinelearn}
The basic principle of machine learning is to train algorithms with data sets in order to improve these algorithms and enable them to extract information about the data automatically \cite[part 1.1]{Wekacourse}. Generally, the goal of machine learning models is to use the underlying input data to predict a certain outcome \cite[part 1.1]{Wekacourse}. For example, if you let run an algorithm over some weather data you may want the algorithm to learn, based on certain attributes like temperature and atmospheric pressure, what weather corresponds with these conditions. Thus, trying to train the algorithm to identify the correct weather based on new input data. In order to properly conduct a machine learning analysis the data set needs to be divided in a training set and a test set where the training set is used to train the algorithm while the test set is used to validate the predictive power of the algorithm \cite[part 2.7]{Wekacourse}. This is absolutely crucial as a validation on the training set would always result in a perfect predictive power of the algorithm. The methods which exist to divide a data set into training and test set and the justification for the use of the 10-Fold Cross-Validation in the present survey is explained in detail in chapter \ref{chap:machinelearning}. 

While all MLAs try to predict the likelihood of a certain attribute based on the input values of other attributes, some algorithms additionally provide insights about the relationship of other attributes with the attribute you are trying to predict. These algorithms are of interest for the present study as it is not the objective to merely predict the likelihood of a certain attribute occurring in an additional paper, but to uncover relationships between attributes that are not necessarily straight forward. However, it must be taken into consideration that the MLAs can solely show correlations between attributes but never causality. 

	
		\subsubsection{Data-Mining}
		\label{subsec:datamin}
While machine learning uses algorithms data-mining merely attempts to extract information and knowledge from a large amount of data by identifying patterns \cite{Datamining17}. In data-mining there is no predefined algorithm which is trained and improved by the data set. Thus, data-mining uses the recognized patterns to build its own predictive model to explain the attributes in a data set \cite{Datamining17}. Hence, machine learning is based on the concept of data mining and combines it with specified algorithms that are trained in the process. 

In order to conduct a data-mining analysis that follows a standardized process, the Cross-Industry Standard Process for Data Mining (CRISP-DM) was developed \cite{crisp-dm2}, \cite{crisp-dm}. The process is divided into 6 phases: Business Understanding (definition of the objectives), Data Understanding (data collection and first examination), Data Preparation (preparation of the final data set), Modeling (application of appropriate data-mining techniques such as MLAs), Evaluation and Deployment (analysis, interpretation and deployment of the results)\cite{crisp-dm2}, \cite{crisp-dm}. Figure \ref{img:crisp-dm} shows the CRISP-DM and all its phases. The phases do not necessarily have to be implemented in this exact sequence and can be executed multiple times \cite{crisp-dm2}, \cite{crisp-dm}. The machine learning analysis conducted in this survey follows the CRISP-DM approach: Objectives are defined, data is collected during the literature review, the collected data is prepared for the WEKA application, MLAs and parameter settings are applied to the data set and the results are evaluated and interpreted.


\begin{figure} [h]
	\centering
	\includegraphics[scale=0.4]{figures/crisp-dm.png}
	\caption{Phases of the CRISP-DM Process Model for Data Mining \cite{crisp-dm2}}
	\label{img:crisp-dm}
\end{figure}

		
		\subsubsection{Algorithms}
		\label{subsec:algo}
The MLAs applied in the present survey belong to the category of classification algorithms. In the present survey the simple classification algorithms J48 and OneR are utilized and benchmarked against the baseline accuracy (ZeroR). The reason why these algorithms are selected is that the J48 algorithm generates a comprehensible decision tree and the OneR algorithm attempts to find the strongest relation between two attributes. Thus, these algorithms are not merely generating a probability for a tested attribute, but additionally provide information about attribute relations. Part of these relations will be evaluated in chapter \ref{chap:machinelearning}. A more detailed explanation of the algorithms applied to the literature review data set of the present survey is covered in chapter \ref{chap:machinelearning} as well.
		
		
		
		
		


==> kapitel/Framework.tex <==
\section{Framework for Predictive Maintenance}
\label{chap:framework}

\begin{figure}[h]
	\centering
	\includegraphics[width=\textwidth]{figures/framework.png}
	\caption{Categories of the Framework for Predictive Maintenance}
	\label{img:framework}
\end{figure}

In section \ref{sec:frameworkconstruction} the methodical approach for structuring the framework was explained. The analysis of the papers resulted in a grid which consists of a total of 69 different attributes. The framework that is built from this data grid is described in the following sections. The entire framework for PM consists of 10 categories. These categories are Goals, Condition Monitoring, Maintenance Scope, Degradation Process, Fault Detection, System Size, Scheduling, Prognostic Techniques, Data Handling and Evaluation. Figure \ref{img:framework} shows these 10 categories which represent the highest level of the framework. The following sections of chapter \ref{chap:framework} describe the categories in detail and show all the attributes which are summarized within a certain category. All figures in chapter \ref{chap:framework} are created by the author of the present survey. For the complete grid data set used to construct the framework for PM see appendix A.

	\subsection{Goals}
	\label{sec:goals}

\begin{figure}[h]
	\centering
	\includegraphics[width=\textwidth]{figures/goals.png}
	\caption{Overview of the Category Goals}
	\label{img:goals}
\end{figure}	

The category of goals is generally used by researches to support their motivation for choosing the research topic of PM. Thus, 139 out of 150 papers (93\%) mention one or several goals of the framework. During the analysis of the paper 8 goals have been identified: Spare Part Inventory Reduction, Prolong Machine/Component Life, Cost Minimization, Minimize Downtime, Availability, Productivity, Reliability and Safety. Some of these goals were already introduced in section \ref{sec:improvements} but not explained in detail. Figure \ref{img:goals} shows all attributes belonging to the category of goals. The number in parentheses is the frequency of occurrence of a certain attribute out of a total of 150 papers. An overview of the entire data grid for the category goals can be found in appendix A.1.

First, PM has the potential to reduce the number of spare parts in stock since a reliable PM system would allow for the possibility to merely store the spare parts needed soon instead of storing every spare part which could potentially be necessary \cite{Zhou2007}. Hence, the PM system would reduce the number of spare parts in stock and the overall storage size while still maintaining a proper maintenance process and avoiding production downtime due to unavailable spare parts.   

Second, some researchers argue that PM can in fact prolong the overall life of machines and components \cite{Wu2007}. This is because the PM system monitors the health condition and predicts the remaining useful life of a machine and thus reduces the risk of a fatal breakdown which might reduce the lifespan of the machine even in case of a thoroughly corrective maintenance action \cite{Wu2007}. Furthermore, as PM systems also help to avoid unnecessary maintenance actions this can additionally prolong a machine's life because every maintenance action puts the machine to risk since a maintenance action and replaced components represent an intervention in the structure of a machine \cite{Baidya2015}.

The by far most frequently mentioned goal is the objective to minimize costs through a PM approach \cite{Deloux2009}. More than two thirds of the analyzed papers mention cost minimization as one of the main goals of PM and thus their research. The goal of cost minimization is often related to other goals of a PM system such as minimizing downtime by avoiding fatal breakdowns or prolong machine life and reduce the need for spare part inventory. As a reliable PM system leads to an overall more efficient way of the maintenance process this results in an overall reduction of costs. Hence, while the implementation of a PM system is costly and complex it is argued to be a positive business case in the long run \cite{Deloux2009}.

Fourth, since PM systems allow fault detection in the future based on monitoring data and prognostic techniques the number of fatal breakdowns can be reduced \cite{Kaiser2009}. With a conventional scheduled maintenance policy based on historic data about the life span of a machine or component, there is still the possibility that a machine or component might fail before the next maintenance interval since the interval is merely an average that includes outliers. In contrast to that, a PM approach monitors the machine and its components regularly or even continuously and triggers maintenance actions regardless of the time a machine or component is in use \cite{Mobley02}. Additionally, a PM system can also minimize the downtime of a manufacturing line as it allows to plan maintenance actions ahead and group certain maintenance actions to reduce the number of production stops for single maintenance actions \cite{Yang2008}. Minimizing downtime has a severe effect on reducing costs and increasing productivity. Thus, almost half (47\%) of the papers in this survey address the objective of minimizing downtime.  

The goals of availability, productivity and reliability are all connected to the goals of cost minimization and minimizing downtime \cite{Raza2017}, \cite{Okoh2017}, \cite{Baidya2015}. By decreasing downtime a PM system automatically increases the total amount of time a machine can be in an online state. The increased overall manufacturing time also increases the productivity of a manufacturing plant as more products can be produced in the same time while the monitoring component of the PM system always makes sure that the equipment is running in a healthy condition. Hence, the PM approach keeps machinery in a state where it produces products in a good quality \cite{Carnero2006}. Thus, this leads to an increase in productivity. The goal to increase the reliability of machines is strongly related to the goal availability as these two objectives are always addressed together. Additionally, availability, productivity and reliability increase the output and quality in a certain time interval and therefore minimize production costs.

Finally, safety is a goal that is not directly related to business performance indicators such as productivity and costs. Nevertheless, it is still an important objective in the context of PM research since it is addressed by almost a third (30\%) of all papers in the present survey. At present, most production lines still require the interaction of humans and are not fully automated. Therefore, humans work nearby or directly with heavy machinery. Fatal breakdowns and unreliable running conditions of these machines cause a potential risk to the employees. Hence, as PM avoids fatal breakdowns and monitors the health condition of machines, the safety of employees is improved \cite{Efthymiou2012}.


	\subsection{Condition Monitoring}
	\label{sec:conditionmonitoring}

\begin{figure}[h]
	\centering
	\includegraphics[width=\textwidth]{figures/conditionmonitoring.png}
	\caption{Overview of the Category Condition Monitoring}
	\label{img:conditionmonitoring}
\end{figure}	

A PM approach is based on the collection of data from a machine or component which indicates its health status and allows the prediction of the residual useful life based on this monitoring data \cite{Gebraeel2005}. The analysis of the 150 papers has identified 4 different attributes for the category of condition monitoring: Inspection-Based Monitoring, Sensor-Based Monitoring, Continuous Monitoring and Online/Real Monitoring. All attributes and their corresponding frequency of occurrence are shown in figure \ref{img:conditionmonitoring}. Furthermore, an overview of the entire data grid for the category condition monitoring can be found in appendix A.2. 

First, the least addressed approach to monitor a machine's condition and collect valuable data is inspection-based monitoring (16\%). With inspection-based monitoring the data is merely collected in inspection intervals. However, the intervals are not predefined as it is the case in conventional maintenance policies. The intervals are adapted with respect to the observed and collected data about a machine's or component's current and predicted conditional state \cite{Jardine2006}. 

Second, since advancements in sensor technology make sensors for various types of parameters more affordable, the majority of studies base their research on sensor-based monitoring. With sensor-based monitoring different types of sensors for instance to observe vibration and temperature are used to collect the relevant data \cite{Orhan2006}. Note that sensor-based monitoring and inspection-based monitoring are not mutually exclusive as it is often the case that sensor equipment is necessary to perform the inspection \cite{Kaiser2009}. Generally, the usage of sensor-technology is more appropriate for an integrated PM system as it is crucial for efficient continuous monitoring.

As the term already indicates, continuous monitoring is the continual collection of relevant monitoring data to estimate the remaining useful life of a machine or component \cite{Traore2015}. In contrast to inspection-based monitoring the amount of data collected is significantly higher since inspection-based monitoring is merely a periodic snapshot of a machine's conditional state. Hence, inspection-based monitoring and continuous monitoring are the only two attributes in this category which are mutually exclusive. All other attribute combinations are feasible.    

Finally, online/real monitoring is a condition monitoring technique which allows the collection of data in the running state of a machine and is addressed by the majority of the analyzed papers (61\%) \cite{Lindstrom2017}. Furthermore, it is the prerequisite for continuous monitoring as a continual collection of data is merely feasible in the running state of a machine. Therefore, researchers always address online monitoring when implementing a continuous monitoring approach in their studies. However, online monitoring is also possible for inspection-based methods, but in this case it does not resemble a requirement.


	\subsection{Maintenance Scope}
	\label{sec:maintenancescope}
	
\begin{figure}[h]
	\centering
	\includegraphics[width=\textwidth]{figures/maintenancescope.png}
	\caption{Overview of the Category Maintenance Scope}
	\label{img:maintenancescope}
\end{figure}	

The category of maintenance scope is a category which is generally not addressed frequently. Obviously, for every maintenance action there has to be an assumption about the maintenance scope but merely a few studies (13\%) mention this category directly. Therefore, the framework solely represents the number of times the topic of maintenance scope is addressed directly. The present survey makes no assumptions about the maintenance scope in cases where no maintenance scope is mentioned directly. The analysis of the papers revealed 3 different attributes for the category maintenance scope: Perfect Maintenance, Imperfect Maintenance and Grouping Maintenance Actions. Figure \ref{img:maintenancescope} shows all attributes belonging to the category of maintenance scope. An overview of the entire data grid for the category can be found in appendix A.3.

First, the attribute of perfect maintenance is based on the assumption that every maintenance action conducted at a machine or component restores the functionality and durability to its original level. Hence, into the condition of a new machine \cite{Dieulle2001}. This assumption follows an \emph{as good as new} approach for every maintenance action \cite{Dieulle2001}. In contrast to this approach, the assumption of imperfect maintenance is based on the premise that a maintenance action cannot restore the functionality and durability of a certain machine into an \emph{as good as new} state, but only into an \emph{as good as old} condition \cite{Tan2010}. Thus, the machine or component is still assumed to be in the state of used equipment even after maintenance. More studies make the assumption of imperfect maintenance compared to perfect maintenance since they argue that it is a more realistic conjecture \cite{Zhou2007}. Generally, the category of maintenance scope is not very widespread in the PM research, presumably because the usually continuous monitoring and prediction updates make the assumption about the maintenance scope obsolete.

The third and final attribute of the category of maintenance scope seems to be far more important for PM but is as well not severely represented in the academic literature. The possibility to group maintenance actions in an efficient way leads to an overall cost reduction for maintenance activities as downtime can be reduced \cite{Ladj2016}, \cite{Nguyen2017}. Precondition for grouping maintenance actions is a holistic PM approach which monitors the entire manufacturing equipment simultaneously in order to identify certain maintenance actions which are best conducted at the same time \cite{Nguyen2017}. While the assumptions about perfect and imperfect maintenance are mutually exclusive, the attribute of grouping maintenance actions can be addressed in combination with the other two attributes of the category. The issue that merely a few of the analyzed papers address the important attribute of grouping maintenance will be discussed in chapter \ref{chap:discussion}.

	
	\subsection{Degradation Process}
	\label{sec:degradationprocess}

\begin{figure}[h]
	\centering
	\includegraphics[width=\textwidth]{figures/degradationprocess.png}
	\caption{Overview of the Category Degradation Process}
	\label{img:degradationprocess}
\end{figure}	
	
The category degradation process is addressed by a third (34\%) of the analyzed papers and covers either the direct modeling of the degradation process of a machine or a predefined assumption about its deterioration course. The attributes identified for this category are: Degradation Modeling, Exponential Degradation Assumption, Random Failure Assumption, Linear Degradation Assumption and Weibull Distribution Assumption. Figure \ref{img:degradationprocess} shows the category degradation process and all its attributes. An overview of the entire data grid for the category can be found in appendix A.4.

First, the process of degradation modeling is the derivation of the deterioration course of a machine or component based on relevant machine health indication data such as vibration or temperature \cite{Gebraeel2006}. The reason for this procedure is to gather information about a certain machines typical conditional state over its lifetime \cite{Gebraeel2006}. The modeling of the deterioration process is beneficial in a sense that having knowledge about a machine's degradation pattern can support a PM system to predict future breakdowns more accurately. Nevertheless, the PM approach is not meant to merely rely on the average degradation of a machine to decide on the maintenance intervals. The main indicator is still the PM system and its prognostic approach that could be supported by the information of the degradation modeling. Figure \ref{img:degradationmodeling} shows an example for an vibration-based degradation course where phase I represents the non-defective state and phase II the conditional state close to failure \cite{Gebraeel2006}. Thus, the objective is to model these phases in order to support the machinery prognostics of the PM decision with regard to the timing and need for maintenance activities.

\begin{figure}
	\centering
	\includegraphics[scale=1]{figures/degradationmodeling.png}
	\caption{Vibration-based Degradation Modeling \cite{Gebraeel2006}}
	\label{img:degradationmodeling}
\end{figure}	

A few papers make an assumption about the degradation process instead of following a modeling approach. However, since the PM approach is based on monitoring the conditional state and prognostics, the mere assumption about the deterioration course of a machine is not really relevant for a PM approach. Hence, only a fraction of the academic literature mentions such an assumption prior to the implementation of an PM approach. The assumptions about linear degradation, exponential degradation and random failure are straight forward \cite{Elwany2008}, \cite{Gebraeel2005}, \cite{Hashemian2011a}. A PM approach would be most efficient in the prsence of random failure since conventional maintenance policies would fail most of the time. Additionally, the academic literature mentions a distribution called Weibull Distribution \cite{Gebraeel2005}. It is a continuous probability distribution based on adjustable parameters which is used to model the lifespan of machines or components \cite{Gebraeel2005}.

	
	\subsection{Fault Detection}
	\label{sec:faultdetection}
	
\begin{figure}[h]
	\centering
	\includegraphics[width=\textwidth]{figures/faultdetection.png}
	\caption{Overview of the Category Fault Detection}
	\label{img:faultdetection}
\end{figure}	
	
A pure PM approach solely focuses on the prediction of the future conditional state of machinery and components to schedule maintenance activities in an appropriate way and scope.  Nevertheless, a little bit over a third (36\%) of the examined academic papers additionally address the topic of fault detection, meaning that the PM approach does not only attempt to predict the remaining useful life of the machine, but also tries to identify the root cause of the failure based on the collected data \cite{Yam2001}. The category of fault detection includes the following attributes: Root Cause Analysis, Machinery Diagnostics and No Fault Detection. All attributes are shown in figure \ref{img:faultdetection}. An overview of the entire data grid for the category fault detection can be found in appendix A.5.

Fault detection covers the additional function of diagnostics. Thereby, root cause analysis and machinery diagnostics address the same issue. While most researchers call it machinery diagnostics, some also refer to it as root cause analysis or mention both terms. The general idea is the processing of acquired monitoring data to uncover the reasons for future failure. Thus, using vibration or other machine monitoring data for diagnostic purposes \cite{DeFaria2015}. The feasibility and accuracy of a fault detection approach depends on the level of monitoring activity which means that the more machine parts and components are monitored separately, the better can be identified where the root cause for a future failure may lie \cite{DeFaria2015}. 

	
	\subsection{System Size}
	\label{sec:systemsize}

\begin{figure}[h]
	\centering
	\includegraphics[width=\textwidth]{figures/systemsize.png}
	\caption{Overview of the Category System Size}
	\label{img:systemsize}
\end{figure}		
	
Another relevant parameter which was identified during the literature review is the category of system size. This category addresses the extent to which the PM approach is applied or assumed to be applied when implemented in real life. The analysis revealed two attributes: Single-Component Systems and Multi-Component Systems. Furthermore, the attribute of multi-component systems is further divided in the sub category of component dependencies which are divided into the following attributes: Structural Component Dependence, Economic Component Dependence and Stochastic Component Dependence. Figure \ref{img:systemsize} shows all attributes of the category. An overview of the entire data grid for the category can be found in appendix A.6. A little bit over two thirds (70\%) of the papers analyzed in the present survey address the category of system size. Hence, this category can be seen as important in the context of PM.

First, single-component systems are defined by the present survey as either single components, e.g. experimental studies which conduct laboratory tests with merely single bearings, or single machines considered solely in an isolated context \cite{Hashemian2011}. This means that the machine itself might consist of multiple components but the total machine as a whole is not considered as a true multi-component system. The definition chosen for this category results in less true multi-component systems compared to single-component systems (61\% vs. 39\%).

As already described in the previous paragraph, the true multi-component system consists of multiple machines or separate components which together form or are part of larger system, e.g. an entire manufacturing line \cite{VanHorenbeek2013}. The implementation of an successful PM system is much more complicated for these multi-component systems since more data needs to be processed and dependencies between the system's components become relevant \cite{VanHorenbeek2013}.  However, while there is a significant number of papers addressing multi-component systems, merely 8 of the 41 papers (20\%) additionally address the topic of dependence. 

Dependence in multi-component systems can be divided in three different types. First, economic dependencies are such dependencies that enable cost reduction when parts of the system are maintained simultaneously, e.g. because for the maintenance of one component other components have to be offline as well, thereby reducing downtime when maintenance actions for these components are conducted jointly \cite{Nguyen2015}. Second, stochastic dependencies are dependencies in consequence of stochastic relations between components of their deterioration process. Hence, the degradation of one component affects the state of one or multiple other components of the system \cite{Nguyen2015}. Finally, structural dependencies result from components which form a unified part in a sense that the maintenance of one component directly implies the maintenance of all structural dependent components \cite{Nguyen2015}. The most important of these three types of dependencies seems to be the economic dependence as all papers which cover the topic of dependence at least mention this type. Furthermore, the existence of these dependencies is the reason why single-component PM approaches are not simply scalable to a multi-component level but must be adapted with regard to the affects of these dependencies \cite{Nguyen2015}.

	
	\subsection{Scheduling}
	\label{sec:scheduling}
	
\begin{figure}[h]
	\centering
	\includegraphics[width=\textwidth]{figures/scheduling.png}
	\caption{Overview of the Category Scheduling}
	\label{img:scheduling}
\end{figure}


The category of scheduling is addressed by almost two third (62\%) of the papers and therefore has an important role in the field of PM. This does not seem to be unusual as the main motivation behind a PM approach is to identify the need and timing for maintenance activities in advance, allowing for an efficient scheduling of these activities. The attributes identified in this category are: Dynamic Action Scheduling, (Autonomous) Dynamic Spare Part Availability and No Scheduling Included. Figure \ref{img:scheduling} shows all attributes of the category and their corresponding frequency of occurrence. An overview of the entire data grid for the category scheduling can be found in appendix A.7. 

First, dynamic action scheduling describes the possibility to dynamically adapt the maintenance schedule based on new and processed condition monitoring data \cite{Yang2008}. This dynamic scheduling is only possible in a PM environment due to the forecast of a machine's future conditional state. Optimization algorithms can be applied to define the most cost-effective maintenance schedule and continuously update this schedule when new machinery prognostics information becomes available \cite{Yang2008}. Hence, the maintenance schedule is not static as it would be for conventional maintenance policies but rather dynamic. 

Additionally, a few papers cover the attribute of (autonomous) dynamic spare part availability, where not only the maintenance activities itself but also the necessary spare part ordering is linked to the PM system \cite{Nguyen2017}. This broader and more integrated approach better fits a modern idea of Industry 4.0 and smart factory compared to an isolated policy. However, over a third (38\%) of the analyzed academic literature does not address the category of scheduling in conjunction with PM  directly.  


	\subsection{Prognostic Techniques}
	\label{sec:prognostictechniques}

\begin{figure}[h]
	\centering
	\includegraphics[width=\textwidth]{figures/prognostictechniques.png}
	\caption{Overview of the Category Prognostic Techniques}
	\label{img:prognostictechniques}
\end{figure}


The category of prognostic techniques is clearly one of the most important ones for PM. While all the monitoring and data acquisition is indispensable the prognostic technique is what transforms the raw data into valuable information. Note that since a prognostic technique attempts to predict a prospective failure of a machine or component the generated information are just probabilities. For the PM framework of the present survey 3 attributes were identified for the category of prognostic techniques: Data-Driven Approach, Model-Based Approach and No Prognostic Approach specified. Figure \ref{img:prognostictechniques} shows all 3 primary attributes as well as their secondary attributes and their corresponding frequency of occurrence. An overview of the entire data grid for the category prognostic techniques can be found in appendix A.8 and A.9.

The analysis of the 150 papers showed that the number and diversity of different techniques is enormous. The majority of techniques is often found only once or twice within all the papers. Thus, the present survey will not present and discuss the different techniques in detail. In addition, the attribute no prognostic approach specified is added to the PM framework since not every paper mentions the applied approach. For the cases in which the papers mention their approach there is no single definition of how to classify these techniques into the attributes data-driven and model-based. Furthermore, some papers just mention that they apply some kind of model-based or data-driven approach but do not specify this approach further, which makes it difficult to stick to one definition for all papers.  

It is important to take into consideration that all these prognostic techniques rely on monitoring data for their predictions. Hence, in a broad sense all these methods are somehow data-driven. However, in the present survey data-driven approaches are such techniques which rely heavily on previous data input in order to enable reliable predictions in the first place \cite{Yuan2013}, \cite{Datadriven11}. Good examples are (multiple) linear regression, logistic regression, regression trees, random forest and the kriging statistical technique. All these techniques are based on the concept of regression \cite{Datadriven11}. However, for a reliable regression model there must be a huge amount of training data to define the model before it can actually be applied to new test data. The same holds for bayesian-based models. Prior to work with the bayesian principle of believe updates the a priori probabilities must be derived from training data \cite{Datadriven11}. 

Beside these classical statistic methods the attribute data-driven approach also has a sub attribute category of prognostic techniques related to artificial intelligence. Almost 25\% of the papers mention an artificial intelligence approach. Most frequently the concept of artificial neural networks. Artificial intelligence concepts also belong to the group of data-driven approaches since they require an enormous amount of training data, too \cite{Kandukuri2016}, \cite{Wu2007}. In the case of an artificial neural network nodes which are also called neurons are structured in multiple layers where every neuron passes on a value to all nodes in the next layer \cite{Ann00}, \cite{Ann02}. Every value is weighted by some real number that represents the weight of the connection between two neurons \cite{Ann00}, \cite{Ann02}. The idea of the network is that a specific input results in a specific outcome with a certain probability \cite{Ann00}, \cite{Ann02}. The network mostly depends on the weights of every connection. However, finding these weights is no easy task and requires a huge amount of training data in order to build a reliable artificial neural network \cite{Ann00}, \cite{Ann02}. In total 73\% of the 124 papers which mention a prognostic technique, mention a data-driven approach.

As already mentioned, the difference between data-driven and model-based approaches is not straightforward but rather vague. Generally, a data-driven prognostic technique is based on a large amount of available historic monitoring data while a model-based technique is applied for new or untested systems which lack this comprehensive measurement data \cite{Yuan2013}. Furthermore, about 8\% of the papers mention both the data-driven and the model-based approach. In the PM framework of the present survey model-based approaches are defined as techniques which process monitoring data but do not require a great amount of training data before they can be applied. However, the allocation of techniques into this attribute is vague and often based merely on the fact that a method does not fit the definition of a data-driven approach properly. Furthermore, the framework shows that about a third (31\%) of the papers apply a model-based approach but the frequencies of the sub attributes are very low. This is the case since a lot of the papers in the model-based attribute merely mention the usage of some type of model for the machinery prognostics part. Thus, even more making the allocation within this framework category a vague process. However, the main purpose of this category is not to find a generally valid classification of every single prognostic technique as this is not feasible, but to demonstrate the variety and number of techniques identified after analyzing just 150 papers of the research area of PM. 


	\subsection{Data Handling}
	\label{sec:datahandling}

\begin{figure}[h]
	\centering
	\includegraphics[width=\textwidth]{figures/datahandling.png}
	\caption{Overview of the Category Data Handling}
	\label{img:datahandling}
\end{figure}

The category data handling deals with the amount of data acquired by condition monitoring. Especially in cases of continuous monitoring with multiple sensors the amount of data collected by these sensors results in an enormous amount of data to be handled \cite{Munirathinam2014}, \cite{Yan2017}. The analysis of the 150 papers covered in the present survey reveals the following relevant attributes: Data Fusion, Data Filtering, Storage Location and Data Access. Additionally, the attributes of storage location and data access are divided into the sub attributes of Local Date Storage and Remote/Cloud Data Storage as well as Local Data Access and Remote Data Access. Figure \ref{img:datahandling} shows all attributes of the category and their corresponding frequency of occurrence. An overview of the entire data grid for the category data handling can be found in appendix A.10. 

First, data fusion and data filtering are two methods which deal with the issue of big data generated by continuous monitoring. The approach of data fusion utilizes the idea to integrate multiple data sources in order to generate more reliable data compared to any individual data source. In case of sensor-generated data, data fusion combines the data of multiple sensors and the resulting more reliable and more accurate data is then processed and analyzed \cite{Kandukuri2016}, \cite{Lee2006}. On the other hand, data filtering also deals with the issue of large amounts of data by filtering uninformative data \cite{Yamato2017}. For the most part continuous monitoring will generate data which just shows that a certain machine is in a normal state \cite{Wang2016}. Therefore, data filtering models identify the useless data and only analyze the informative parts of the total amount of data, thus making the data processing more accurate and efficient \cite{Schirru2010}. However, merely the minority (14\%) of the papers directly address either data fusion, data filtering or both.

Second, in contrast to data fusion and filtering, data storage and access are attributes addressed by all papers. This is the case since every paper includes some type of monitoring which inevitably generates data that needs to be stored and made accessible for further processing. The analysis shows that for both, storage location and data access, the remote alternative is chosen by only about 20\% of the papers and mostly in combination with IoT, Industry 4.0 and cloud computing \cite{Chiu2017}, \cite{Yan2017}, \cite{Lee2006}. This fact is of interest as the remote approach seems to be more suitable for an efficient PM system in an Industry 4.0 environment, especially with a manufacturing structure that consists of multiple production sites. Hence, the method of remote storage and access is not covered as much as expected in the recent academic literature. This issue will be discussed in chapter \ref{chap:discussion} of the present survey.


	\subsection{Evaluation}
	\label{sec:evaluation}

\begin{figure}[h]
	\centering
	\includegraphics[width=\textwidth]{figures/evaluation.png}
	\caption{Overview of the Category Evaluation}
	\label{img:evaluation}
\end{figure}

Finally, the framework of the present survey for PM is concluded by the category of evaluation. This category covers the application-oriented part of the studies. Most of the studies use some sort of data to test their PM approach and to proof its feasibility. The following attributes were identified for this category: (Numeric) Simulation, Evaluation based on Real Data, Experiment and Comparison with Conventional Maintenance Policies. Figure \ref{img:evaluation} shows all attributes of the category and their corresponding frequency of occurrence. An overview of the entire data grid for the category evaluation can be found in appendix A.11.

Note that none of the attributes are mutually exclusive. Nevertheless, only 6 papers out of 150 choose a combination of numeric simulation and either real data or experiment. First, the numeric simulation is an evaluation based merely on simulated date, e.g. a Monte Carlo Simulation which generates data about hypothetical failures which must then be identified by the researcher's PM approach \cite{DeSaporta2012}, \cite{Lei2015a}. More than a third (37\%) of the papers apply a simulation-based evaluation method to test their PM techniques. Second, 37\% of the papers choose an evaluation based on real data. For this evaluation method the researchers acquire actual data from companies who monitor their machines \cite{Schmidt2017}, \cite{Elwany2008}. The data includes the monitoring data as well as information about the corresponding state of the machine, e.g. whether a failure occurred. This data can then be used to validate the accuracy and performance of the introduced PM approach. The advantage of real data is that it allows to test the PM approach with long term data and with data gathered from multiple large and complex machines. 

In contrast to that, the minority of papers (13\%) conducts experiments to validate their approach. Mostly, the experiments are kept very small in a sense that merely one component, e.g. bearings or a detached engine are used as experimental subjects \cite{Gebraeel2005}, \cite{Yang2002}. Thus, experiments are usually limited to small scaled test setups which makes them unsuitable to validate approaches that include multi-component systems and dependencies as well as connections with other related processes. Finally, about 20\% of the authors additionally compare their PM approach with conventional maintenance policies as a benchmark. These comparisons are generally based on comparing total costs for different maintenance policies including the PM approach \cite{VanHorenbeek2013}, \cite{Nguyen2015}. Thus, attempting to prove the superior efficiency and cost reduction opportunities of PM.


==> kapitel/Introduction.tex <==
\section{Introduction}
\label{chap:introduction}
Maintenance has always been a severe cost driver in the production industry. Studies show that depending on the industry between 15 and 70 percent of total production costs originate from maintenance activities \cite{You2010}. Nevertheless, the majority of the production industry still relies on outdated maintenance policies and focuses on an inefficient run to failure approach or statistical trend driven maintenance intervals \cite{Mobley02}.Thus, leading to reduced production time and product quality as a result of inappropriate maintenance policies. According to \cite{Mobley02} surveys on maintenance show that about 33 cents of every dollar spent on maintenance in the US is wasted because of unnecessary maintenance activities. On the other hand, comprehensive research with regard to modern maintenance policies using modern technologies is conducted in different fields of academics such as computer science, production and artificial intelligence. The usage of well-developed sensors and prognostic techniques allows a relatively reliable prediction of the remaining useful life of plant equipment. This so-called Predictive Maintenance (PM) policy is especially of interest in the environment of Industry 4.0 and severely enhances the efficiency of modern production facilities. The main benefits of PM are presented in the following section \ref{sec:improvements}.  
  

	\subsection{Improvements through Predictive Maintenance}
	\label{sec:improvements}
Predictive maintenance is based on the idea that certain characteristics of machinery can be monitored and the gathered date be used to derive an estimation about the remaining useful life of the equipment. Hence, this kind of maintenance policy implicates several important improvements in the manufacturing and maintenance process which can severely reduce production costs \cite{Grall2002}. First, PM can reduce the number of unnecessary maintenance activities as it is not based on periodic maintenance intervals bound to average lifetime. Thus, potentially reducing the overall number of maintenance activities over a machine's life. Second, not only can too early maintenance activities be avoided, but also too late activities as equipment might fail before the next periodic maintenance interval since the intervals rely on average lifetime which likely includes significant positive but also negative deviations from the mean. For example, due to the specific structure in which a certain component is deployed in larger machinery. Both, the reduction of unnecessary maintenance as well as the reduction of fatal breakdowns result in increased productivity and reduced production down time. Therefore, depending on the accuracy of the prognostic method applied, PM can be considered as an overall improvement of efficiency in contrast to conventional maintenance policies \cite{Nguyen2015},\cite{Yam2001}. These and further improvements and goals of PM approaches are presented in chapter \ref{chap:framework}. 


	\subsection{Objectives and Research Questions}
	\label{sec:objectives}
The existing research on predictive maintenance is comprehensive and dates back decades with still hundreds of new published papers annually \cite{Jardine2006}. Nevertheless, as the environment is changing and new technologies become available at a more affordable price, there is still a wide range of potential for new research in the field of PM. Especially in the context of the Internet of Things (IoT) and Industry 4.0 the possibilities to integrate PM and connect it to other systems of the production process are increasing. In order to identify the potential starting points for further research the objective of the present survey is to structure the complex of themes regarding PM and to put the comprehensive amount of research into a transparent and comprehensible framework. Thus, leading to the first research question of the present survey: How can predictive maintenance approaches be differentiated and classified?

Additionally the present survey integrates a machine learning tool called WEKA into the process of analyzing the data retrieved from the academic literature review. Machine learning classification algorithms are applied for this purpose. Hence, the second research question is: Can Machine Learning Algorithms (MLAs) improve the informational value of a survey? 

	
	\subsection{Methodical Approach}
	\label{sec:methodicalapproach}
The methodical approach of the the present survey is a Structured Literature Review (SLR) based on the keywords \emph{Predictive Maintenance}. Thereafter, all relevant attributes of the selected papers are inserted in an Excel table which is utilized to construct the framework and to conduct the machine learning analysis. A detailed description of the methodical procedure and the necessary preparations for building the framework and conducting the machine learning analysis with WEKA is described in chapter \ref{chap:procedure}. 	
	
	
	\subsection{Structure of the Thesis}
	\label{sec:structure}
The remainder of the survey is structured as follows: Chapter \ref{chap:foundations} includes the theoretical principals and foundations of PM and machine learning. It also puts PM in the context of IoT and Industry 4.0. Next, chapter \ref{chap:procedure} describes the methodical procedure of the literature review, the framework construction and the machine learning analysis. Chapter \ref{chap:framework} explains in detail the categories and the most important attributes of the PM framework. Subsequently, chapter \ref{chap:machinelearning} covers the actual machine learning analysis and the explanation and selection process of the applied MLAs for classification purposes. In chapter \ref{chap:discussion} follows a discussion of the framework and machine learning analysis results in context of the objectives and research questions introduced in section \ref{sec:objectives}. Finally, chapter \ref{chap:conclusion} concludes the survey by summarizing the main findings, critically reviewing the work and giving recommendations for future research.




==> kapitel/Machine-Learning.tex <==
\section{Machine Learning Analysis}
\label{chap:machinelearning}
The following chapter covers the machine learning analysis part of the present survey. As already introduced in section \ref{sec:machinelearn} machine learning tries to find and learn correlations from training data in order to be able to predict the characteristic of a certain attribute \cite[part 1.10]{Wekacourse} (see the weather example in section \ref{sec:machinelearn}). In the present survey a software tool called WEKA is used to apply machine learning to the data acquired from analyzing the 150 papers. For this purpose the data grid with all the papers and ticked attributes is transformed into a data grid where each cell for every instance is filled with either true when a certain attribute is covered in the paper or false if this is not the case. Each row in the data grid represents a paper and is called an instance. Additionally, the Excel file is transformed into an ARFF file via a CSV format. However, as mentioned in section \ref{sec:machinelearn} the objective of the present survey is not to predict true or false for a certain attribute for new papers, but to discover relationships between attributes. Therefore, the simple classifier MLAs applied in this survey are the ZeroR, OneR and J48 algorithm. While ZeroR is used as baseline accuracy the other algorithms offer additional information about the relationships between attributes bedsides merely resulting in a probability for predicting the tested attribute in new instances \cite[part 2.12]{Wekacourse}. Of course, WEKA offers more simple MLAs like the Naive-Bayes algorithm. However, e.g. Naive-Bayes makes the assumption that all attributes are equally important and statistically independent which is exactly the opposite of what the survey tries to reveal \cite[part 3.7]{Wekacourse}. The MLAs ZeroR, OneR and J48 are applied to all 69 attributes of the PM framework as well as the attributes year, publication type and whether the paper is a survey. A brief explanation for every algorithm as well as the results are covered in section \ref{sec:zeror}, \ref{sec:oner} and \ref{sec:j48}. In order to perform a machine learning analysis the data set has to be divided in a training set and a test set \cite[part 2.7]{Wekacourse}. The methods for this step are described in section \ref{sec:dataset}.

When working with machine learning and data mining software the developers of WEKA advise to be mindful about the following aspects. First, always try to keep your analysis, the algorithms and parameter settings as simple as possible and avoid over-engineering \cite[part 3.4]{Wekacourse}. Second, data mining is an experimental science. There is no right or wrong nor is there a universal best MLA \cite[part 5.2]{Wekacourse}. Third, be cautious about interpreting the results, as machine learning is solely able to reveal correlation but no causality \cite[part 5.7]{Wekacourse}. Finally, be cautious about overfitting. This issue is discussed in more detail in section \ref{sec:overfitting}.


\subsection{Training and Test Data Set}
\label{sec:dataset}
If there are no multiple data sets available the first step in a machine learning analysis will be to divide the single data set into a training data set and a test data set. This is important since an evaluation of a MLA on the data it was trained with would always result in a perfect fit. The most obvious approach is the hold-out method where the data set is divided by a single percentage split, e.g. 90\% of the data are used for training and 10\% of the data are used for testing \cite[part 2.7]{Wekacourse}. The majority of the data set should always be used for training in order to provide the algorithm with sufficient learning opportunity \cite[part 2.7]{Wekacourse}. However, as the data set in the present survey contains merely a total of 150 instances the percentage split is not suitable as characteristics might solely be represented in the test or training set \cite[part 2.14]{Wekacourse}. The cross validation method offers a solution for the drawback of a mere percentage split and is therefore applied in the machine learning analysis of the present survey. Cross validation divides the data set based on a random number generator in a predefined number of equally large sub sets \cite[part 2.14]{Wekacourse}. Thereafter, always all sub sets except for one are used for training the chosen MLA and the remaining sub sets are used for testing it \cite[part 2.14]{Wekacourse}. This process is repeated until every subset was used as test set once. The results of the runs are then averaged \cite[part 2.14]{Wekacourse}. Thus, cross validation reduces the variance of the output and is especially functional for small data sets as it is basically a repeated hold-out \cite[part 2.14]{Wekacourse}. WEKA uses 10-Fold Cross Validation as standard, meaning that the data set is divided into 10 equally large sub sets. 10-Fold Cross Validation is also applied in the analysis of the present survey. There is no proper reason for using 10-Fold Cross Validation other then the fact that always 90\% and thus a large amount of the data set are used for training \cite[part 2.14]{Wekacourse}. To sum it up, the possible methods are a separate data set, testing on the training data set (not advisable), hold-out and cross validation. For the described reasons cross validation is applied from this point forward.



\subsection{Baseline Accuracy (ZeroR)}
\label{sec:zeror}
The ZeroR algorithm is also called the baseline accuracy and cannot be seen as a proper MLA. The simple idea behind ZeroR is to decide about an attributes presumable value based on the characteristic with the highest frequency in the data set \cite[part 2.12]{Wekacourse}. Thus, in the case of a mere true or false possibility for an attribute's value, the algorithm chooses the one with the highest frequency and tests in how many cases this decision would be correct. For example, if a specific prognostic technique happens to be true for only 3 papers then the algorithm would choose always false when deciding whether this prognostic technique appears in an instance and would be correct in 98\% with regard to the entire data set. Therefore, the algorithm would choose false for every new instance based on this probability \cite[part 2.12]{Wekacourse}. Hence, the learning process is solely based on frequency of occurrence. This is the reason why ZeroR is used as a benchmark for other more complex algorithms in order to compare their performance to the simple ZeroR procedure. Note that for the ZeroR algorithm no split into training and test data set is conducted. Table \ref{tab:zeror} shows an extract of the results for the ZeroR algorithm. The entire overview for all 72 tested attributes can be found in appendix B.1. Since the attribute year is a numeric attribute instead of a nominal one, the ZeroR algorithm cannot be applied. Note that these results are only used as a reference and not as an elimination criterion for the validity of other algorithms, as the objective of the analysis is not to achieve the highest percentage, but to reveal relations between attributes. Nevertheless, the baseline accuracy can be applied as an indicator for the significance of the potential relationships found by the other algorithms.

\begin{table}
\centering
\begin{tabular}{|clc|}
\hline
ID & Attribute Name & ZeroR in\% \\
\hline
01 & Year &	n/a		\\
02 & Publication Type & 67,33	\\
03 & Survey & 93,33	\\
04 & Availability & 52,67	\\
05 & Reliability & 52,67	\\
06 & Safety	& 70,00	\\
07 & Productivity &	66,00	\\
08 & Spare Part Inventory Reduction & 82,67	\\
09 & Cost Minimization & 69,33	\\
10 & Minimize Downtime & 52,67	\\
11 & Prolong Machine/Component Life & 80,67	\\
12 & No Goals Mentioned & 92,67	\\
13 & (Numeric) Simulation & 62,67	\\
14 & Experimental Evaluation & 87,33	\\
. & . & . \\
. & . & . \\
. & . & . \\
19 & Grouping Maintenance Actions & 95,33	\\
20 & Inspection-Based Monitoring & 84,00	\\
21 & Sensor-Based Monitoring & 60,00	\\
22 & Online/Real Time Monitoring & 61,33	\\
23 & Continuous Monitoring & 71,33	\\
. & . & . \\
. & . & . \\
. & . & . \\
35 & Logistic Regression & 98,67	\\
. & . & . \\
. & . & . \\
. & . & . \\
61 & Single-Component System & 57,33	\\
62 & Multi-Component System & 72,67	\\
63 & Economic Component Dependence & 94,67	\\
64 & Structural Component Dependence & 98,00	\\
65 & Stochastic Component Dependence & 96,67	\\
66 & Multi-Component Systems without Dependencies & 78,00	\\
67 & Data Fusion & 94,00	\\
68 & Data Filtering & 92,00	\\
69 & Local Data Storage & 84,00	\\
70 & Remote/Cloud Data Storage & 84,00	\\
71 & Local Data Access & 80,00	\\
72 & Remote Data Access & 80,00	\\
\hline
\end{tabular} 
\caption{Extract of Results of the ZeroR Algorithm}
\label{tab:zeror}
\end{table}

\subsection{OneR Algorithm}
\label{sec:oner}
The first MLA which is not based solely on the frequency of occurrence is the OneR algorithm. The ZeroR algorithm does not intend to base its decision about true or false on other than the attributes frequencies itself. Thus, no relations with other attributes are considered. In contrast to ZeroR, the OneR algorithm bases the decision about the tested attribute on one other attribute \cite[part 3.2]{Wekacourse}. Since every attribute except for year and publication type can only take the value true or false, the OneR algorithm tries to find the best attributed which explains the characteristic of the tested attribute based on merely these two nominal characteristics, e.g. according to OneR the attribute single-component system (ID 61) can be best explained by the attribute experimental evaluation (ID 14). Hence, when ID 14 is true (false) then ID 61 is true (false) as well in over 60\% of the cases. In this case the OneR algorithm achieves an accuracy of 63.33\% (see table \ref{tab:oner}) while the baseline accuracy (ZeroR) of ID 61 is merely 57.33\%. Note that the absolute value of the percentage outcome cannot be interpreted generally \cite[part 2.12]{Wekacourse}. An outcome of 99\% does not necessarily has to be good and vice versa for an outcome of merely 50\%. The results indicate that there might be a connection between these two attributes. A plausible hypothesis for the result could be that experimental set-ups are often small and do not allow to test for complex multi-component systems consisting of multiple machines. Thus, the OneR algorithm supports the finding of relationships such as the one described and is therefore a suitable algorithm for the objectives of the present survey. Table \ref{tab:oner} shows an extract of the results for the OneR algorithm. An overview over the entire list of attributes can be found in appendix B.2. The column Relation represents the direction of the relationship between the OneR attribute and the tested attribute. For example t$\rightarrow$ f/f$\rightarrow$ t means that if the OneR attribute is true the tested attribute is false and vice versa. The attribute survey (ID 2) is a special case since it does not merely consist of the values true and false. Thus, the c in the relation column stands for conference and the j for journal.  For the analysis of every attribute the parameter settings for the OneR algorithm are kept to the default settings advised by the developers of WEKA. 

The OneR algorithm cannot find an explanatory attribute for 22 of the 72 attributes. Additionally, no attributes were removed from the list for the analysis for a certain sub group of attributes in order to avoid a distortion of the results. Furthermore, holding the number of attributes constant also allows to compare all results. This would not be the case if the attributes for certain tests were different. Furthermore, the OneR algorithm is not informative for attributes with a low frequency of occurrence since in most cases where no OneR attribute could be found the tested attribute has a relatively low frequency. Finally, a problem with the OneR algorithm occurs when attributes mutually explain each other. An example are local data access (ID 71) and remote data access (ID 72). 

The presumable relation between ID 61 and ID 14 was already presented. Another attribute relationship found by the OneR algorithm occurs between grouping maintenance actions (ID 19) and economic component dependence (ID 63). Whenever ID 63 is true (false), ID 19 happens to be true (false) as well in 98\% of the cases. Even though the delta between the ZeroR predictive power and the OneR predictive power is merely 1.34\%, the relationship is still plausible since the potential cost savings with respect to economic dependencies can be realized by grouping maintenance actions. On the other hand, since the algorithm tries to generate the best fit based on mere statistics, there are also unexpected outcomes such as the OneR relation between continuous monitoring (ID 23) and logistic regression (ID 35). As already described in section \ref{sec:conditionmonitoring} continuous monitoring can only be achieved if online monitoring is feasible. Hence, the expectation would be that online/real time monitoring (ID 22) is the OneR attribute for continuous monitoring. Nevertheless, although ID 35 only appears in 2 instances it still achieves the better result for ID 23 compared to the more obvious ID 21. Obviously, the relation between the two attributes seems to be merely a coincidence, especially with regard to the low frequency of ID 35. Thus, be cautious when interpreting the results of the analysis. An detailed evaluation similar to the previous examples for every attribute is out of the scope of the present survey. Nevertheless, all necessary information for an evaluation of attributes of interest can be found in appendix B.2. Appendix B.2 only lists the attribute ID but all the corresponding attribute names can be found in appendix B.1 which shows the complete results of the ZeroR analysis.

\begin{table}
\centering
\begin{tabular}{|ccccc|}
\hline
ID & OneR in \% & OneR Attribute (ID) & Relation & $\Delta$ to ZeroR in \%  \\
\hline
01 & n/a & n/a & n/a & n/a \\
02 & 68,67 & 29 & t$\rightarrow$ c/f$\rightarrow$ j & 1,34 \\
03 & 94,67 & 35 & t$\rightarrow$ t/f$\rightarrow$ f & 1,34 \\
04 & 100,00 & 05 & t$\rightarrow$ t/f$\rightarrow$ f & 47,33 \\
05 & 100,00 & 04 & t$\rightarrow$ t/f$\rightarrow$ f & 47,33 \\
06 & 74,00 & 08 & t$\rightarrow$ t/f$\rightarrow$ f & 4,00 \\
07 & 68,67 & 69 & t$\rightarrow$ f/f$\rightarrow$ t & 2,67 \\
08 & 90,00 & 59 & t$\rightarrow$ t/f$\rightarrow$ f & 7,33 \\
09 & 76,67 & 12 & t$\rightarrow$ f/f$\rightarrow$ t & 7,34 \\
10 & 62,67 & 62 & t$\rightarrow$ t/f$\rightarrow$ f & 10,00 \\
11 & 81,33 & 34 & t$\rightarrow$ t/f$\rightarrow$ f & 0,66 \\
12 & 93,33 & 45 & t$\rightarrow$ t/f$\rightarrow$ f & 0,66 \\
13 & 72,00 & 15 & t$\rightarrow$ f/f$\rightarrow$ t & 9,33 \\
14 & 88,00 & 34 & t$\rightarrow$ t/f$\rightarrow$ f & 0,67 \\
. & . & . & . & . \\
. & . & . & . & . \\
. & . & . & . & . \\
19 & 96,67 & 63 & t$\rightarrow$ t/f$\rightarrow$ f & 1,34 \\
20 & 85,33 & 32 & t$\rightarrow$ t/f$\rightarrow$ f & 1,33 \\
21 & 70,67 & 22 & t$\rightarrow$ t/f$\rightarrow$ f & 10,67 \\
22 & 70,67 & 21 & t$\rightarrow$ t/f$\rightarrow$ f & 9,34 \\
23 & 72,67 & 35 & t$\rightarrow$ t/f$\rightarrow$ f & 1,34 \\
. & . & . & . & . \\
. & . & . & . & . \\
. & . & . & . & . \\
35 & n/a & n/a & n/a & n/a \\
. & . & . & . & . \\
. & . & . & . & . \\
. & . & . & . & . \\
61 & 63,33 & 14 & t$\rightarrow$ t/f$\rightarrow$ f & 6,00 \\
62 & 94,67 & 66 & t$\rightarrow$ t/f$\rightarrow$ f & 22,00 \\
63 & 98,00 & 65 & t$\rightarrow$ t/f$\rightarrow$ f & 3,33 \\
64 & 98,67 & 65 & t$\rightarrow$ t/f$\rightarrow$ f & 0,67 \\
65 & 98,67 & 64 & t$\rightarrow$ t/f$\rightarrow$ f & 2,00 \\
66 & 94,67 & 62 & t$\rightarrow$ t/f$\rightarrow$ f & 16,67 \\
67 & 95,33 & 35 & t$\rightarrow$ t/f$\rightarrow$ f & 1,33 \\
68 & 92,67 & 46 & t$\rightarrow$ t/f$\rightarrow$ f & 0,67 \\
69 & 100,00 & 70 & t$\rightarrow$ f/f$\rightarrow$ t & 16,00 \\
70 & 100,00 & 69 & t$\rightarrow$ f/f$\rightarrow$ t & 16,00 \\
71 & 100,00 & 72 & t$\rightarrow$ f/f$\rightarrow$ t & 20,00 \\
72 & 100,00 & 71 & t$\rightarrow$ f/f$\rightarrow$ t & 20,00 \\
\hline
\end{tabular} 
\caption{Extract of Results of the OneR Algorithm}
\label{tab:oner}
\end{table}


\subsection{J48 Algorithm}
\label{sec:j48}
The second fully adequate MLA used in this analysis is the J48 algorithm. The J48 algorithm is different form OneR as it considers more than merely one attribute in order to predict the characteristics of the tested attribute \cite[part 3.9]{Wekacourse}. J48 is especially useful for the objective of the present survey to reveal relationships between attributes since it generates comprehensible decision trees. The algorithm produces an percentage outcome as performance measurement for the predictive power of the model as well. Nevertheless, the outcome is also presented in form of an easily understandable decision tree \cite[part 3.9]{Wekacourse}. The principle of the J48 algorithm follows a top-down induction, more precisely a recursive divide and conquer strategy to generate the decision tree \cite[part 3.9]{Wekacourse}. Explaining this methodology in detail is out of scope of this survey. Detailed information regarding this topic can be found in the WEKA video course created by the software's developers \cite[part 3.9]{Wekacourse}. Relevant for the present survey is the fact that the J48 algorithm produces the smallest tree with the purest nodes \cite[part 3.9]{Wekacourse}. The most relevant parameter setting for the J48 decision trees is called pruning. Pruning deals with controlling the size of the nodes and whether to split nodes further and create a larger tree \cite[part 3.11]{Wekacourse}. The intention behind pruning is that the model might not fit the training data as good as possible anymore, but at the same time makes the tree more general and therefore more informative outside the scope of the training data \cite[part 3.11]{Wekacourse}. Additionally, the trees get smaller when pruning is applied. In WEKA there is a parameter called Minimum Number of Objects. The parameter requires a minimum number of instances inside the last node and avoids a further split if this would result in a shortfall of this threshold \cite[part 3.11]{Wekacourse}. For the analysis of the present survey the parameter for the minimum number of objects was raised from its default value of 2 to 5. The reason for the increase is to control the size of the trees since the large number of 72 attributes partially produces massive trees for a pruning value of 2. Nevertheless, be cautious about pruning as it could also result in overfitting since it not only can result in more general models, but also more specific models tailored to the training data \cite[part 3.11]{Wekacourse}.The issue of overfitting is discussed in section \ref{sec:overfitting}.  

An extract of the results are shown in table \ref{tab:j48}. An overview of the results for every attribute can be found in appendix B.3. Appendix B.3 only lists the attribute ID but all the corresponding attribute names can be found in appendix B.1 which shows the complete results of the ZeroR analysis. Note that the J48 algorithm cannot produce a decision tree for every attribute, especially when the frequency of occurrence for the tested attribute is low. This is the case for 28 out of the 72 attributes. The output for these 28 attributes is the same percentage as for the ZeroR algorithm.

In order to compare the result of the two algorithms OneR and J48 the same attributes are evaluated in this section. As for the results of the OneR algorithm it is out of scope of the present survey to discuss the results for every tested attribute in detail. The entire output of the J48 algorithm including every decision tree can be found in appendix B.3 and C. Hence, all information to evaluate any specific attribute of interest is available. Figure \ref{img:treeid61_2} shows the J48 decision tree for the attribute ID 61. It becomes visible that even with a pruning parameter setting of 5 the trees can still become large and complex. The leafs of the tree either contain one or two values. The first value is the number of right choices based on the model and the second value represents the number false choices. For example, if experimental evaluation (ID 14) is true then the algorithm suggests that ID 61 is true as well. This is true for 15 instances but wrong for 1 instance. Since multiple leafs lead to errors when selecting true or false, the percentage predictive power of the algorithm is below 100\%. In this case 65.33\%. It is interesting that the J48 tree does not has ID 14 (the OneR attribute) as its top attribute but in third place. Thus, the two attributes related to component dependencies (ID 65 and ID 66) seem the be relevant as well as the experimental evaluation attribute. This seems to be consistent since component dependencies would require a multi-component instead of a single-component system. Hence, as the J48 algorithm is not limited to one attribute it is likely to reveal more relevant attribute relations compared to the OneR algorithm. However, although the J48 tree is large, complex and involves a total of 12 attributes it outperforms the simple OneR algorithm consisting of just one attribute by merely 2\%.

For attributes which are mutually exclusive such as ID 71 and 72 the J48 algorithm produces the same output as the OneR algorithm and generates a tree consisting of merely one attribute which is similar to the OneR attribute (see figure \ref{img:treeid71_2}). The same holds for attributes which are not perfectly explained by another attribute but relatively close to a perfect fit. Since the the model does not require the decision tree to generate entirely pure nodes the leafs can contain mistakes. Therefore, for these attributes the J48 algorithm again results in the same outcome as the OneR algorithm although (see figure \ref{img:treeid19_2} for ID 19 and 63). 

The strength of the J48 algorithm becomes visible when comparing the results for continuous monitoring (ID 23). Figure \ref{img:treeid23_2} shows the tree for ID 23 and the first attribute of the tree is online/real time monitoring which would be expected since it is the requirement for continuous monitoring. Additionally, the algorithm bases its decision on the attribute multi-component system (ID 62). This implies that continuous monitoring is especially used in a system where multiple machines have to be monitored simultaneously. Hence, continuous monitoring seems to be an efficient solution for such comprehensive PM systems. In contrast to the informative result of the J48 algorithm, the OneR algorithm based its model on a prognostic technique which appears in merely 2 instances.

To sum it up, the J48 algorithm is a reliable and robust MLA which generates an comprehensible decision tree \cite[part 3.9]{Wekacourse}. While the OneR algorithm is simple and reveals one presumable attribute relation, the J48 algorithm is able to detect more complex  interactions based on multiple attributes. If interested in a specific attribute one can get a first impression based on the OneR result but should always take the additional effort to evaluate the J48 tree in order to get a deeper understanding of possible attribute relations.   

\begin{figure}
	\centering
	\includegraphics[width=\textwidth, height=\textheight]{figures/treeid61.png}
	\caption{J48 Decision Tree for Single-Component System (ID 61)}
	\label{img:treeid61_2}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=\textwidth]{figures/treeid71.png}
	\caption{J48 Decision Tree for Local Data Access (ID 71)}
	\label{img:treeid71_2}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=\textwidth]{figures/treeid19.png}
	\caption{J48 Decision Tree for Grouping Maintenance Actions (ID 19)}
	\label{img:treeid19_2}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=\textwidth, height=\textheight]{figures/treeid23.png}
	\caption{J48 Decision Tree for Continuous Monitoring (ID 23)}
	\label{img:treeid23_2}
\end{figure}

\begin{table}
\centering
\begin{tabular}{|cccc|}
\hline
ID & J48 Tree generated & J48 in \% & $\Delta$ to ZeroR in \%  \\
\hline
01 & no & n/a & n/a \\
02 & yes & 60,00 & -7,33 \\
03 & no & n/a & n/a \\
04 & yes & 100,00 & 47,33 \\
05 & yes & 100,00 & 47,33 \\
06 & yes & 74,00 & 4,00 \\
07 & yes & 65,33 & -0,67 \\
08 & yes & 90,00 & 7,33 \\
09 & yes & 72,67 & 3,34 \\
10 & yes & 61,33 & 8,66 \\
11 & yes & 79,33 & -1,34 \\
12 & yes & 93,33 & 0,66 \\
13 & yes & 80,00 & 17,33 \\
14 & yes & 86,00 & -1,33 \\
. & . & . & . \\
. & . & . & . \\
. & . & . & . \\
19 & yes & 96,67 & 1,34 \\
20 & yes & 80,00 & -4,00 \\
21 & yes & 63,33 & 3,33 \\
22 & yes & 75,33 & 14,00 \\
23 & yes & 76,00 & 4,67 \\
. & . & . & . \\
. & . & . & . \\
. & . & . & . \\
35 & no & n/a & n/a \\
. & . & . & . \\
. & . & . & . \\
. & . & . & . \\
61 & yes & 65,33 & 8,00 \\
62 & yes & 100,00 & 27,33 \\
63 & yes & 95,33 & 0,66 \\
64 & yes & 98,00 & 0,00 \\
65 & yes & 98,00 & 1,33 \\
66 & yes & 100,00 & 22,00 \\
67 & no & n/a & n/a \\
68 & no & n/a & n/a \\
69 & yes & 100,00 & 16,00 \\
70 & yes & 100,00 & 16,00 \\
71 & yes & 100,00 & 20,00 \\
72 & yes & 100,00 & 20,00 \\
\hline
\end{tabular} 
\caption{Extract of Results of the J48 Algorithm}
\label{tab:j48}
\end{table}


\subsection{Overfitting}
\label{sec:overfitting}
A severe issue in machine learning is the problem of overfitting \cite[part 3.4]{Wekacourse}. Overfitting is defined as the state in which a MLA fits the training data too tight \cite[part 3.4]{Wekacourse}. Hence, the algorithm is not general enough. Overfitting can occur when a large number of different algorithms with different parameter settings are tested for a certain attribute until the best fit is found \cite[part 3.4]{Wekacourse}. The process is then repeated for every attribute tested in the machine learning analysis. There will always be a combination for which an algorithm fits the input data for a certain attribute almost perfectly \cite[part 3.4]{Wekacourse}. However, the objective of machine learning is not to find the algorithm that fits the input data best. In order to avoid the issue of overfitting in the present survey, the applied algorithms as well as their parameter settings are defined prior to the analysis and held constant for every attribute. Nevertheless, there should be cautiousness about overfitting even in presence of the described countermeasures.




==> kapitel/Methodology.tex <==
\section{Methodical Procedure}
\label{chap:procedure}
The following chapter describes the methodology used to select the relevant papers, construct the framework and conduct the machine learning analysis with the data mining tool WEKA. In section \ref{sec:review} the SLR method is explained which is used to select the relevant papers. Additionally, the method is compared to another approach called berry picking and it is discussed why a SLR is considered to be the more suitable method for the topic of PM. In total 150 papers are selected to derive the framework and conduct the machine learning analysis. Section \ref{sec:frameworkconstruction} describes the construction of the PM framework for which the 150 papers are investigated in detail to fill an Excel table with all the relevant attributes concerning the topic of PM. Thereafter, all the attributes are clustered into 10 categories that build the main layer of the framework. Finally, section \ref{sec:machineapproach} concludes the methodology part by introducing the machine learning part of the present survey.


	\subsection{Structured Literature Review}
	\label{sec:review}
The Structured Literature Review (SLR) is a systematic approach to find the relevant literature in order to answer a set of research questions by searching for papers based on predefined key words \cite{Slr14}. By searching with specific key words the method allows to find the most relevant literature to address the research questions. However, there is no guarantee that a SLR is able to find all relevant literature \cite{Slr14}. Nevertheless, the SLR has the advantage to tackle a specified topic from numerous directions, allowing the researcher to properly cover the important sub themes \cite{Slr14}. Thereby, the SLR allows to uncover gaps in the existing primary research and helps to reveal areas where additional research might be needed \cite{Slr14}.

As the field of predictive maintenance is extremely broad and has been addressed comprehensively by researchers for decades, the existing pool of papers is enormous. Therefore, the only key words used in the present survey to detect the relevant literature with a Google Scholar search are \emph{Predictive Maintenance}. As the objective of the survey is to construct a framework addressing the distinctive facets of PM this procedure results in the most favorable set of important literature since a combined search of PM and Industry 4.0 mainly results in papers which address Industry 4.0 but only mention PM as part of it without explaining a specific approach in detail. Thus, with these papers the development of a detailed framework with all facets of PM would not be possible. As already mentioned, the tremendous amount of research addressing the topic of PM results in thousands of potentially relevant papers which cannot be evaluated in a single survey. Thus, the present survey does not claim to be entirely complete and only represents an overview. The search algorithm of Google Scholar runs very successful as the first papers of the search are the most suitable papers for the topic, while the quality and usefulness of the later papers is steadily decreasing. This allows to identify appropriate literature by checking the list of results from the top down. The search for academic papers via Google Scholar was conducted in October 2018. A paper for the framework was selected by first scanning the abstract to identify the detail in which the topic of PM is covered in the paper. If a paper is explaining the applied PM approach and its context, e.g. system size and condition monitoring in detail, it is utilized to build the framework. A complete list of the 150 papers classified for building the framework can be examined in appendix A. The selected papers are published between 1993 and 2018 while almost two thirds (97/150) are published during the last decade. Since the research concerning PM is a very broad field it is addressed by various types of journals and conferences.

Another literature review method that was considered for the present survey is the so-called berry picking method. In this method the review starts by identifying a starting paper that matches the addressed topic and objectives \cite{berry08}. The following step in the process is the footnote chasing where the list of references of the starting paper is checked for more relevant literature \cite{berry08}. Furthermore, the search for relevant literature can be extended by checking not only the references of the starting paper, but also checking the papers which cite the starting paper \cite{berry08}. The drawback of this method is that the papers are most likely connected based on a similar sub theme that is addressed by these papers, thereby potentially missing important other subsections of the main topic. Of course, this issue can be approached by choosing multiple starting papers to cover the missing sub themes. Nevertheless, the amount of literature addressing PM is so broad and contains numerous sub themes that even with an increased number of starting papers the berry picking method would still miss relevant fields. Hence, the SLR is considered as better method for the present survey as it allows to find more diversified relevant literature in order to cover a much broader scope of the topic. Thus, resulting in a more favorable result for building the framework and addressing the first research question specified in section \ref{sec:objectives}. 

	
	\subsection{Construction of the Framework}
	\label{sec:frameworkconstruction}
The construction of the framework starts by examining the first paper that was selected from the top down of the potentially relevant literature of the Google Scholar search. Notice that it is not important with which paper this process is started as the whole process has an iterative characteristic. While a paper is examined a table is filled with data about the relevant attributes covered in the paper. Thus, whenever an important attribute or characteristic concerning the topic of PM is identified a new column is added to the table and the attribute is ticked for this paper. Thereafter, every paper that is categorized in the table gets a separate line to mark the attributes which are covered in this paper. Thereby, the following papers are checked iteratively as their research content is searched for the already existing attributes. Additionally, the following papers are checked for additional relevant attributes which are added to the table. The data grid that is generated by this process represents the foundation of the PM framework. It is important to mention that an attribute is merely considered as covered by a paper if it is a direct research subject of the paper. Hence, a literature review within a primary study is not considered sufficient to fulfill certain attributes. However, the list of categorized papers also contains 10 surveys (\cite{Jardine2006}, \cite{Lee2006}, \cite{DeFaria2015}, \cite{Efthymiou2012}, \cite{Edwards1998}, \cite{Heng2009}, \cite{Kandukuri2016}, \cite{Lu2009}, \cite{Munirathinam2014}, \cite{Muller2008}) where the approach is obviously different and all referenced attributes are marked in the table.

In the next step the raw data grid is structured by grouping attributes which are similar to each other or belong to the same sub theme. Subsequently, each cluster is named by a term which represents the content of the cluster. These umbrella terms build the main categories of the framework. If appropriate, the clusters can have further subdivisions to allow for a finer classification within the categories. Thus, the entire framework can be best represented in form of a tree. The main categories of the PM framework, as well as the tree structure for every category are presented in chapter \ref{chap:framework}.
	
	
	\subsection{Machine Learning Approach}
	\label{sec:machineapproach}
As already mentioned in chapter \ref{sec:objectives} the present survey also contains a machine learning part in order to analyze the relevant attributes of the data grid. Thus, checking for relationships between the attributes which cannot be detected easily. The main objective is to identify whether a machine learning analysis of literature review data is useful in a sense that it allows an improved evaluation of the academic literature by identifying these potential attribute connections. Thereby, reaching a deeper understanding of the topic and to examine hypotheses about PM and its attributes.

The basics about machine learning and the purpose of MLAs have already been explained in section \ref{sec:machinelearn}. The tool or machine learning software that is used for the present survey is called Waikato Environment for Knowledge Analysis (WEKA). It was developed by the University of Waikato and offers a variety of machine learning techniques and algorithms \cite{Wekacourse}. WEKA is written in Java, platform-independent and is an open source software \cite{Wekacourse}.  

As WEKA needs all the data in form of an Attribute-Relation File Format (ARFF) the data table needs to be transformed. First, all columns which only serve as identification, e.g. title and author are removed, leaving only the columns year of publication, whether the paper is a survey, the publication type and all the topic related PM attributes. Additionally, every cell must be filled with either true or false, respectively. In the original grid a certain attribute was merely ticked, leaving the majority of the cells blank. Subsequently, the modified Excel table is saved in a Comma-Separated Values (CSV) format and then rewritten in the editor into an ARFF file structure. The basic structure of an ARFF file is shown in \cite{Wekacourse}. The ARFF file is then used to analyze the data in WEKA by running the simple classification MLAs ZeroR, OneR and J48. The explanation of these algorithms as well as the reason for their selection in contrast to other algorithms is described in detail in chapter \ref{chap:machinelearning}.


